Artemis: Structured Visual Reasoning for Perception Policy Learning

Recent reinforcement-learning frameworks for visual perception policy usually incorporate intermediate reasoning chains expressed in natural language. Empirical observations indicate that such purely linguistic intermediate reasoning often reduces performance on perception tasks. We argue that the core issue lies not in reasoning per se but in the form of reasoning: while these chains perform semantic reasoning in an unstructured linguistic space, \textbf{visual perception requires reasoning in a spatial and object-centric space}. In response, we introduce \textbf{Artemis}, a perception-policy learning method that performs structured visual reasoning, where each intermediate step is represented as a (label, bounding-box) pair capturing a verifiable visual state. This design enables explicit tracking of intermediate states, direct supervision for proposal quality, and avoids ambiguity introduced by language-based reasoning. Building upon verifiable and spatially grounded reasoning chains, Artemis provides a unified architecture for diverse perceptual tasks, without requiring the task-specific designs relied upon by prior perceptual policy models. Trained using grounding and detection sampeles in natural image domains, Artemis generalizes to counting and geometric perception tasks. At its core, a spatially grounded, object-centric chain rule provides a principled foundation for scalable and general perceptual policies.

==> tables/ablation_cold_start.tex <==
\begin{table}[t]
\tablestyle{5pt}{1.05}
\caption{Effect of different cold start strategies on grounding and detection performance.}
\begin{tabular}{l|ccc|ccc}
 & \multicolumn{3}{c|}{Visual Grounding (Acc@0.5)} & \multicolumn{3}{c}{COCO2017 Val (mAP)} \\
Cold Start Strategy & RefCOCO & RefCOCO+ & RefCOCOg & mAP & AP$_{50}$ & AP$_{75}$ \\
\shline
No Cold Start (0) &  91.0  &  85.3  &  87.2  &  29.8 & 45.0  &  31.0  \\
5k Grounding Only &  90.6  &  84.5  &  86.2  &  28.5 & 44.5  &  29.0    \\
5k Grd + 5k Det (Balanced) &  90.5  &  84.6  &  86.5  & 29.1 & 45.4  &  29.8  \\
80k Detection Only &  91.3  &  85.3  &  87.3  &  31.0 & 48.0  &  31.9   \\
\hline
\end{tabular}
\vspace{-0.6em}
\label{tab:coldstart}
\vspace{-1.0em}
\end{table}


==> tables/ablation_joint.tex <==
\begin{wraptable}{r}{9.5cm}
\centering
\begin{minipage}{1.0\linewidth}
\scriptsize
\caption{Ablation study comparing different training orders for grounding (Grd.) and detection (Det.) tasks. 
“Det. $\rightarrow$ Grd.” means training detection first, then grounding; 
“Grd. $\rightarrow$ Det.” means training grounding first, then detection; 
“Joint” means training both tasks simultaneously.}
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{1pt}
\tablestyle{16.5pt}{1.2}
\begin{tabular}{l|ccccc}
\shline
\textbf{Training Order} & \textbf{RefCOCOg$_\text{val}$} & \textbf{COCO$_\text{mAP}$} & \textbf{MATHGLANCE} & $\text{\textbf{Pixmo}}_{\texttt{\textbf{val}}}$ & $\text{\textbf{LISA}}_{\texttt{\textbf{test}}}$ \\
\shline
Det. $\rightarrow$ Grd. & 86.9 & 28.4 & 46.7 & 77.1 & 68.8 \\
Grd. $\rightarrow$ Det. & 87.2 & 30.9 & 42.7 & 79.2 & 67.8 \\
\rowcolor{lightgold} Joint & \textbf{87.3} & \textbf{31.0} & \textbf{49.3} & \textbf{81.4} & \textbf{69.8} \\
\shline
\end{tabular}}
% \vspace{-1.8em}
\label{tab:training_order}
\end{minipage}
\end{wraptable}


==> tables/ablation_sft_rl.tex <==
\begin{table}[t]
\caption{Effect of selection of RL or SFT on grounding and detection performance.}
\tablestyle{5pt}{1.05}
\begin{tabular}{l|ccc|ccc}
 & \multicolumn{3}{c|}{Visual Grounding (Acc@0.5)} & \multicolumn{3}{c}{COCO2017 Val} \\
Cold Start Strategy & RefCOCO & RefCOCO+ & RefCOCOg & mAP & AP$_{50}$ & AP$_{75}$ \\
\shline
No SFT and RL &  88.6  &  81.9  & 85.1   &  15.4 & 22.5  & 15.9   \\
SFT-Full &  82.7  & 76.9  & 79.9   & 26.5  & 40.9  &  27.4    \\
SFT-Grd. &  81.8  &  75.9  & 79.6  & 13.7 & 19.8  & 14.4   \\
SFT-Det. &  51.7  & 39.7   & 42.3   & 26.0  & 39.7  & 27.0    \\
Default RL &  91.0  & 85.3   & 87.2   & 29.8  & 45.0  &  31.0   \\
\hline
\end{tabular}

\label{tab:sft_rl}
\vspace{-1.0em}
\end{table}


==> tables/det.tex <==
\begin{wraptable}{r}{9.5cm}
\centering
\begin{minipage}{1.0\linewidth}
\caption{Object detection evaluation on COCO2017 val. Models marked with $^\dagger$ denote results from our own inference. Gray rows indicate expert models (from MMDetection~\cite{mmdetection}).}
\resizebox{1.0\linewidth}{!}{
\tablestyle{5pt}{1.0}
\begin{tabular}{l|ll|ccccc}
\shline
 \multirow{2}{*}{\textbf{Method}}& \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{Epoch}} & \multicolumn{4}{c}{\textbf{Object detection COCO2017 Val}} \\\cline{4-7}
 &  &  & mAP & $\text{AP}_{50}$ & $\text{AP}_{75}$ & AR$_{100}$ \\
\shline

\rowcolor{moonveil}\multicolumn{7}{l}{\textit{Expert Models}}\\
\hline

\rowstyle{\color{dt}}YOLOv3~\cite{yolov3} & \scriptsize \textcolor{gray}{-} & \textcolor{gray}{273} & \textcolor{gray}{27.9} & \textcolor{gray}{49.2} & \textcolor{gray}{28.3} & \textcolor{gray}{-} \\
\rowstyle{\color{dt}}Faster-RCNN~\cite{faster-rcnn} & \scriptsize \textcolor{gray}{-} & \textcolor{gray}{12} & \textcolor{gray}{35.6} & \textcolor{gray}{55.7} & \textcolor{gray}{37.9} & \textcolor{gray}{-} \\


% \rowstyle{\color{dt}}DETR~\cite{detr} & \scriptsize \textcolor{gray}{41M} & \textcolor{gray}{500} & \textcolor{gray}{42.0} & \textcolor{gray}{62.4} & \textcolor{gray}{44.2} & \textcolor{gray}{-} \\
\hline
\rowcolor{moonveil}\multicolumn{7}{l}{\textit{General MLLMs}}\\
\hline
Qwen2.5-VL$^\dagger$~\cite{qwen2.5vl} & \scriptsize 3B & 1 & 15.4 & 22.5 & 15.9 & 29.8 \\
Griffon~\cite{griffon-13b} & \scriptsize 13B & 1 & 24.8 & 40.6 & 25.1 & - \\
\hline
\rowcolor{moonveil}\multicolumn{7}{l}{\textit{RL-based MLLMs}}\\
\hline
VLM-R1$^\dagger$ \cite{vlm-r1} & \scriptsize 3B & 1 & 21.6 & 35.6 & 21.7 & 33.2 \\
Vision-R1 \cite{vision-r1} & \scriptsize 7B & 1 & 26.6 & 40.0 & 27.8 & - \\
Perception-R1 \cite{perception-r1} & \scriptsize 3B & 1 & \textbf{31.9} & 46.7 & \textbf{33.4} & 41.2 \\
\hline
\rowcolor{lightgold}\textbf{Artemis} & \scriptsize 3B & 1 & 31.0 & \textbf{48.0} & 31.9 & \textbf{46.6} \\\shline
\end{tabular}
}
% \vspace{-.5em}

\label{tab:detection}
% \vspace{-1.em}
\end{minipage}
\end{wraptable}


==> tables/zero_shot_perception_math.tex <==
\begin{table*}[!t]\footnotesize
 % \vspace{-.5em}
 \caption{Zero-shot accuracy on MATHGLANCE benchmark. The evaluation covers four types of questions: \textit{cls} (shape classification), \textit{cnt} (object counting), \textit{grd} (object grounding), and \textit{rlat} (relationship identification). \textit{all} indicates the overall accuracy for each subject, while \textbf{Avg.} reports the mean \textit{all} score across all three subjects. Models marked with $^\dagger$ denote results from our own inference.}
 \centering
 \renewcommand\arraystretch{1.2}
 \setlength{\tabcolsep}{1.6mm}{
 \resizebox{1.0\linewidth}{!}{
\begin{tabular}{lc|c|ccccc|ccccc|ccccc}
\shline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{Avg.}} & \multicolumn{5}{c|}{\textbf{Plane  Geometry}} & \multicolumn{5}{c|}{\textbf{Solid  Geometry}} & \multicolumn{5}{c}{\textbf{Graphs}} \\ \cline{4-18} 
 &&& \textit{all} & \textit{cls} & \textit{cnt} & \textit{grd} & \textit{rlat} & \textit{all} & \textit{cls} & \textit{cnt} & \textit{grd} & \textit{rlat} & \textit{all} & \textit{cls} & \textit{cnt} & \textit{grd} & \textit{rlat} \\ \shline
\rowcolor{moonveil}\multicolumn{18}{l}{\textit{General MLLMs}}   \\ \hline
G-LLaVA~\cite{g-llava} &7B& 30.3& 25.6 & 27.8 & 41.2 & 0.4 & 38.0 & 32.3 & 45.4 & 38.1 & 4.8 & 32.5 & 33.9 & 58.0 & 37.0 & 0.0 & 42.4 \\ 
DeepSeek-VL2-Tiny~\cite{deepseekvl2}& 3B& 32.6 & 29.5 & 45.2 & 34.4 & 4.6 & 32.0 & 39.0 & 76.7 & 32.0 & 0.0 & 37.5 & 29.4 & 39.1 & 57.4 & 0.0 & 18.2 \\ 
Qwen2.5-VL$^\dagger$ \cite{qwen2.5vl} & 3B& 33.1 & 31.0 & 42.5 & 22.0 & 20.3 & 38.0 & 37.1 & 75.6 & 33.0 & 0.0 & 30.0 & 31.2 & \textbf{71.0} & 29.6 & 0.0 & 9.1 \\ 
LLaVA-v1.5~\cite{llava1.5} & 7B & 33.3 & 29.2 & 29.0 & 39.6 & 14.2 & 37.5 & 31.6 & 43.0 & 42.3 & 0.0 & 31.3 & 39.0 & 76.8 & 35.2 & 0.0 & 39.4 \\ 

\hline
\rowcolor{moonveil}\multicolumn{18}{l}{\textit{RL-based MLLMs}}   \\ \hline 

VLM-R1$^\dagger$ \cite{vlm-r1} & 3B& 34.4 & 26.9 & 38.0 & 27.6 & 0.7 & 44.0 & 43.6 & 72.1 & 50.5 & 0.0 & 38.8 & 32.6 & 73.9 & 29.6 & 0.0 & 12.1 \\ 
No-Thinking-RL$^\dagger$ \cite{no_think_rl} & 2B& 45.3 & 33.2 & 44.3 & \textbf{44.8} & 0.4 & 46.0 & 56.4 & \textbf{96.5} & 57.7 & 0.0 & 56.3 & 46.3 & 65.2 & 61.1 & 0.0 & 69.7 \\ 
Perception-R1$^\dagger$ \cite{perception-r1}& 2B& 45.3 & 29.7 & 42.5 & 34.0 & 4.3 & 38.5 & \textbf{59.5} & \textbf{96.5} & \textbf{67.0} & \textbf{6.4} & 52.5 & 46.8 & 66.7 & 55.6 & 0.0 & 78.8 \\ 

\hline
\rowcolor{lightgold}\bf Artemis & 3B& \textbf{49.3} & \textbf{39.2} & \textbf{50.6} & 30.4 & \textbf{24.2} & \textbf{52.0} & 56.4 & 93.0 & 53.6 & \textbf{6.4} & \textbf{60.0} & \textbf{52.3} & 65.2 & \textbf{75.9} & \textbf{1.61} & \textbf{81.8} \\ 
\shline
\end{tabular}}}
% \vspace{-1.em}
 
%  \vspace{-1.em}
\label{tab:mathglance}
\end{table*}

==> tables/zero_shot_perception_natural.tex <==
\begin{wraptable}{r}{9.5cm}
\centering
\begin{minipage}{1.0\linewidth}
\caption{Zero-shot visual counting on Pixmo-Count and reasoning grounding on LISA test. Models marked with $^\dagger$ denote results from our own inference. Models marked with $^\ddagger$ follow a detect-then-count paradigm, deriving counts from predicted boxes.}
\resizebox{1.0\linewidth}{!}{
\tablestyle{1.2pt}{1.0}
\begin{tabular}{ll|cccc}
\shline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Size}} &
\multicolumn{2}{c}{\textbf{Visual Counting}} & \multicolumn{1}{c}{\textbf{Reasoning Grounding}} \\ \cline{3-5}
 & & $\text{Pixmo}_{\texttt{val}}$ & $\text{Pixmo}_{\texttt{test}}$ & $\text{LISA}_{\texttt{test}}$ \\
\shline

\rowcolor{moonveil}\multicolumn{5}{l}{\textit{General MLLMs}}\\
\hline
LLaVA-v1.5~\cite{llava1.5} & \scriptsize 7B & 33.3 & 31.0 & - \\
% LLaVA-1.6~\cite{cambrian} & \scriptsize 7B & 32.7 & 31.9 & - \\
LLaVA-OV~\cite{llava-ov} & \scriptsize 7B & 55.8 & 53.7 & - \\
Qwen2-VL~\cite{qwen2vl} & \scriptsize 2B & 60.2 & 50.5 & - \\
Qwen2.5-VL$^\dagger$ \cite{qwen2.5vl} & \scriptsize 3B & 58.0 & 57.8 & 67.4 \\
% Qwen2.5-VL$^\dagger$ & \scriptsize 7B & 71.6 & 72.2 & - \\
\hline
\rowcolor{moonveil}\multicolumn{5}{l}{\textit{RL-based MLLMs}}\\
\hline
VisionReasoner$^\ddagger$\cite{visionreasoner} & \scriptsize 7B & 70.1 & 69.5 & - \\
Perception-R1~$^\ddagger$\cite{perception-r1} & \scriptsize 2B & 78.1 & 75.6 & - \\
UniVG-R1 \cite{univg} & \scriptsize 7B  & - & - & 59.7 \\
No-Thinking-RL \cite{no_think_rl} & \scriptsize 2B  & - & - & 61.8\\
VLM-R1 \cite{vlm-r1}  & \scriptsize 3B  & - & - & 63.1 \\
\hline
\rowcolor{lightgold}\textbf{\mymethod} & \scriptsize 3B & \textbf{81.4} & \textbf{76.92} & \textbf{78.3} \\\shline
\end{tabular}
}
% \vspace{-.5em}

\label{tab:zero_shot_perception_natural}
% \vspace{-1.5em}
\end{minipage}
\end{wraptable}

